CHEX-MATE: Multi-probe analysis of Abell 1689

The nature of the elusive dark matter can be probed by comparing the predictions of the cold dark matter framework with the gravitational field of massive galaxy clusters. However, a robust test of dark matter can only be achieved if the systematic uncertainties in the reconstruction of the gravitational potential are minimized. Techniques based on the properties of intracluster gas rely on the assumption that the gas is in hydrostatic equilibrium within the potential well, whereas gravitational lensing is sensitive to projection effects. Here we attempt to minimize systematics in galaxy cluster mass reconstructions by jointly exploiting the weak gravitational lensing signal and the properties of the hot intracluster gas determined from X-ray and millimeter (Sunyaev-Zel'dovich) observations. We construct a model to fit the multi-probe information within a common framework, accounting for non-thermal pressure support and elongation of the dark matter halo along the line of sight. We then apply our framework to the massive cluster Abell 1689, which features unparalleled multi-wavelength data. In accordance with previous works, we find that the cluster is significantly elongated along the line of sight. Accounting for line-of-sight projections, we require a non-thermal pressure support of $30\text{-}40\%$ at $r_{500}$ to match the gas and weak lensing observables. The joint model retrieves a concentration $c_{200}\sim7$, which is lower and more realistic than the high concentration retrieved from weak lensing data alone under the assumption of spherical symmetry ($c_{200}\sim15$). Application of our method to a larger sample will allow us to study at the same time the shape of dark matter mass profiles and the level of non-thermal pressure support in galaxy clusters.

==> results_table_1.tex <==
\begin{table*}
\caption{Combined Analysis Posterior Distributions: Median Values and $1\sigma$ uncertainties (i.e. posterior distribution between the 16th and 84th percentile).}
\label{table:combined}
\centering

\begin{tabular}{ccccccccccc}
\toprule

Model name & $P_{NT}$ type & $c_{200}$ & $r_{200}$ [kpc] & $M_{200}$ [$10^{15}M_{\odot}$] & $\alpha_{\operatorname{NT}}( \frac{r_{200}}{2})$ & $e$ & $c_{\text{norm}}$ & $r_s$ & $\alpha$ \\
\midrule

\multicolumn{9}{c}{NFW X-ray analysis} \\
\midrule

1-a & None & $6.01^{+0.23}_{-0.24}$ & $2141^{+33}_{-29}$ & $1.30^{+0.06}_{-0.05}$ & x & x & x & x & x \\ 

\midrule
\multicolumn{9}{c}{NFW X-ray and SZ analysis} \\
\midrule

1-b & None & $6.14^{+0.19}_{-0.18}$ & $2188^{+23}_{-22}$ & $1.39^{+0.04}_{-0.04}$ & x & x & x & x & x \\ 

1-c & None & $6.48^{+0.21}_{-0.20}$ & $2039^{+22}_{-23}$ & $1.13^{+0.04}_{-0.04}$ & x & $1.30^{+0.03}_{-0.03}$ & x & x & x \\ 

\midrule
\multicolumn{9}{c}{NFW (1st row) and Einasto (2nd row) weak lensing only analysis} \\
\midrule

2-a  & None & $15.40^{+3.03}_{-3.38}$ & $2298^{+95}_{-81}$ & $1.61^{+0.21}_{-0.16}$ & x & x & x & x & x \\ 

2-b & None & $7.52^{+0.67}_{-1.20}$ & $2593^{+144}_{-167}$ & $2.32^{+0.41}_{-0.42}$ & x & x & $4.07^{+0.61}_{-0.81}$ & $344.7^{+88.5}_{-48.7}$ & $0.17^{+0.12}_{-0.06}$ \\ 

\midrule
\multicolumn{9}{c}{NFW joint X-ray and weak lensing analysis} \\
\midrule

3-a & None & $5.89^{+0.23}_{-0.22}$ & $2165^{+33}_{-30}$ & $1.35^{+0.06}_{-0.06}$ & x & x & x & x & x \\ 

3-b & None & $5.49^{+0.24}_{-0.22}$ & $2154^{+32}_{-29}$ & $1.33^{+0.06}_{-0.05}$ & x & $1.59^{+0.14}_{-0.14}$ & x & x & x \\ 

3-c & Polytropic & $6.60^{+0.72}_{-0.57}$ & $2450^{+81}_{-72}$ & $1.95^{+0.20}_{-0.17}$ & $0.29^{+0.06}_{-0.06}$ & x & x & x & x \\ 

3-d & Angelinelli & $7.20^{+0.35}_{-0.35}$ & $2598^{+66}_{-67}$ & $2.33^{+0.18}_{-0.18}$ & $0.37^{+0.03}_{-0.04}$ & x & x & x & x \\ 

3-e & Polytropic & $5.95^{+0.71}_{-0.47}$ & $2330^{+76}_{-72}$ & $1.68^{+0.17}_{-0.15}$ & $0.19^{+0.07}_{-0.07}$ & $1.35^{+0.18}_{-0.15}$ & x & x & x \\

3-f & Angelinelli & $7.32^{+0.99}_{-0.69}$ & $2624^{+217}_{-150}$ & $2.40^{+0.65}_{-0.39}$ & $0.38^{+0.11}_{-0.09}$ & $0.97^{+0.24}_{-0.27}$ & x & x & x \\ 

\midrule
\multicolumn{9}{c}{NFW joint X-ray, SZ, and weak lensing analysis} \\
\midrule

4-a & None & $6.41^{+0.20}_{-0.22}$ & $2046^{+26}_{-24}$ & $1.14^{+0.05}_{-0.04}$ & x & $1.30^{+0.03}_{-0.03}$ & x & x & x \\ 

4-b & Polytropic & $6.44^{+0.77}_{-0.56}$ & $2369^{+73}_{-71}$ & $1.76^{+0.17}_{-0.15}$ & $0.34^{+0.05}_{-0.06}$ & $1.30^{+0.03}_{-0.03}$ & x & x & x \\ 

4-c & Angelinelli & $7.46^{+0.59}_{-0.49}$ & $2363^{+64}_{-73}$ & $1.75^{+0.15}_{-0.16}$ & $0.30^{+0.04}_{-0.05}$ & $1.30^{+0.03}_{-0.03}$ & x & x & x \\ 

\midrule
\multicolumn{9}{c}{Einasto joint X-ray, SZ, and weak lensing analysis} \\
\midrule

4-d & Polytropic & $5.83^{+0.51}_{-0.63}$ & $2415^{+106}_{-101}$ & $1.87^{+0.26}_{-0.23}$ & $0.36^{+0.05}_{-0.05}$ & $1.30^{+0.03}_{-0.03}$ & $3.12^{+0.41}_{-0.42}$ & $414.6^{+70.9}_{-49.3}$ & $0.21^{+0.03}_{-0.02}$ \\ 

\bottomrule
\end{tabular}

\end{table*}
    
    
